CoherentGS: Sparse Novel View Synthesis with Coherent 3D Gaussians

The field of 3D reconstruction from images has rapidly evolved in the past few years, first with the introduction of Neural Radiance Field (NeRF) and more recently with 3D Gaussian Splatting (3DGS). The latter provides a significant edge over NeRF in terms of the training and inference speed, as well as the reconstruction quality. Although 3DGS works well for dense input images, the unstructured point-cloud like representation quickly overfits to the more challenging setup of extremely sparse input images (e.g., 3 images), creating a representation that appears as a jumble of needles from novel views. To address this issue, we propose regularized optimization and depth-based initialization. Our key idea is to introduce a structured Gaussian representation that can be controlled in 2D image space. We then constraint the Gaussians, in particular their position, and prevent them from moving independently during optimization. Specifically, we introduce single and multiview constraints through an implicit convolutional decoder and a total variation loss, respectively. With the coherency introduced to the Gaussians, we further constrain the optimization through a flow-based loss function. To support our regularized optimization, we propose an approach to initialize the Gaussians using monocular depth estimates at each input view. We demonstrate significant improvements compared to the state-of-the-art sparse-view NeRF-based approaches on a variety of scenes.

==> sec/0_abstract.tex <==
\begin{abstract}
The field of 3D reconstruction from images has rapidly evolved in the past few years, first with the introduction of Neural Radiance Field (NeRF) and more recently with 3D Gaussian Splatting (3DGS). The latter provides a significant edge over NeRF in terms of fast training and real-time inference while improving the reconstruction quality. Although the current 3DGS approach works well for dense input images, the unstructured point-cloud like representation quickly overfits to the more challenging setup of sparse training images (e.g., 3 images), creating a representation that appears as a jumble of needles from novel views. We propose to solve this issue by regularized optimization and depth-based initialization. Specifically, we optimize the Gaussian blobs to smoothly and independently deform different object surfaces to compensate for the inaccuracies of the initialization by utilizing an implicit convolutional decoder and a total variation loss. To support our regularized optimization, we initialize a 3D Gaussian representation from each input view through a novel technique that utilizes monocular depth. We demonstrate significant improvements in terms of recovering scene geometry and texture compared to state-of-the-art sparse-view NeRF-based approaches on a variety of scenes.

\end{abstract}

